Explainable AI for Multivariate Time Series Pattern Exploration: Latent Space Visual Analytics with Temporal Fusion Transformer and Variational Autoencoders in Power Grid Event Diagnosis

Detecting and analyzing complex patterns in multivariate time-series data is crucial for decision-making in urban and environmental system operations. However, challenges arise from the high dimensionality, intricate complexity, and interconnected nature of complex patterns, which hinder the understanding of their underlying physical processes. Existing AI methods often face limitations in interpretability, computational efficiency, and scalability, reducing their applicability in real-world scenarios. This paper proposes a novel visual analytics framework that integrates two generative AI models, Temporal Fusion Transformer (TFT) and Variational Autoencoders (VAEs), to reduce complex patterns into lower-dimensional latent spaces and visualize them in 2D using dimensionality reduction techniques such as PCA, t-SNE, and UMAP with DBSCAN. These visualizations, presented through coordinated and interactive views and tailored glyphs, enable intuitive exploration of complex multivariate temporal patterns, identifying patterns' similarities and uncover their potential correlations for a better interpretability of the AI outputs. The framework is demonstrated through a case study on power grid signal data, where it identifies multi-label grid event signatures, including faults and anomalies with diverse root causes. Additionally, novel metrics and visualizations are introduced to validate the models and evaluate the performance, efficiency, and consistency of latent maps generated by TFT and VAE under different configurations. These analyses provide actionable insights for model parameter tuning and reliability improvements. Comparative results highlight that TFT achieves shorter run times and superior scalability to diverse time-series data shapes compared to VAE. This work advances fault diagnosis in multivariate time series, fostering explainable AI to support critical system operations.

==> Backup/backup.tex <==



%aims to lower the technical barriers and cost to the development of advanced scientific software to facilitate urban and environmental management within smart city initiatives.


 

%This research introduces a system-based methodology to automate the development of sophisticated web-based GIS applications to support urban and environmental management within smart city initiatives. By employing ontology-driven prompts and large language models (LLMs), our approach leverages the AI's capabilities in generation, reasoning, and learning to create a primitive autonomous agent that assists academic researchers and prospective developers by lowering both the technical barriers and costs associated with developing cyberinfrastructure and scientific software tools. Technically, we have developed a prototyping framework that creates a Knowledge Graph (KG) to digitally represent software engineering practices, popular application stacks, package management tools, and domain-specific knowledge of data and simulations. The KG is later used to generate, tune, and enhance engineered prompts through iterative procedures, providing precise instructions for the ChatGPT 4.0 API, DALL-E API, and LangChain to automate the development of geo-visual dashboards using web frameworks and technologies favored by the industry. We demonstrate the effectiveness and feasibility of our framework with a case study of an AI-generated visual dashboard of atmospheric and dispersion data from real-time sensors, machine learning analytics, and environmental simulations using the React framework and Python Tornado server. This study investigates the potential of LLMs to function as full-stack web developers and GIS analysts. By leveraging scientific KGs, the LLMs are guided to comprehend advanced software design and architecture patterns, such as MVC and MVVM, as well as complex scientific data, illuminating the autonomous development of robust, generalized, and scalable geospatial web applications that perform efficiently on both the server and client sides.


%This pipeline leverages urban
%science domain ontologies to transform scientific concepts (datasets, simulation models, metrics, AI algorithms) into software components using robust design patterns. Utilizing LLMs for natural language understanding, reasoning, and coding, it automatically implements these components in popular programming languages. Our AI-powered urban digital twins offer advanced capabilities: real-time IoT data visualization, multi-objective decision optimization, and predictive analytics for urban dynamics. We validate our pipeline with three smart city case studies focusing on freight transportation management, urban climate modeling, and building energy optimization. Implemented using the GPT-4 API in a Python environment, our pipeline synergizes with knowledge graphs created using prevalent ontology languages. The results are compelling: for each case study, the pipeline efficiently generated operational digital twins using an MVC-based Python framework. This marks a significant reduction in manual software design and coding efforts. Our research presents a pioneering path towards next-generation AI-powered urban digital twins that are self-generating, self-organizing, and self-executing, demonstrating the transformative potential of LLMs in urban technology development.



%The study develops 
%The study develops formal models, both information and functional, and establishes the methodological foundations for integrating ontology-driven prompts with ChatGPT's meta-learning capabilities. The resulting productive triad comprises the methodological foundations, advanced information technology, and the OntoChatGPT system, which collectively enhance the effectiveness and performance of chatbot systems. The implementation of this technology is demonstrated using the Ukrainian language within the domain of rehabilitation. By applying the proposed methodology, the OntoChatGPT system effectively extracts entities from contexts, classifies them, and generates relevant responses. The study highlights the versatility of the methodology, emphasizing its applicability not only to ChatGPT but also to other chatbot systems based on LLMs, such as Google's Bard utilizing the PaLM 2 LLM. The underlying principles of meta-learning, structured prompts, and ontology-driven information retrieval form the core of the proposed methodology, enabling their adaptation and utilization in various LLM-based systems. This versatile approach opens up new possibilities for NLP and dialogue systems, empowering developers to enhance the performance and functionality of chatbot systems across different domains and languages.


%Large Language Models (LLMs) have revolutionized fields ranging from creative writing to code generation with their deep understanding of human language. In this paper, we harness the LLMs' capabilities to automate the full-stack web application development of GIS-based scientific visual dashboard to support environmental management and
%smart city research. 

Developing web-based dashboards for advanced querying, visualization, and interaction with GIS data in environmental research often requires repeated, costly software development. While generative AI (GenAI) code generation shows promise, it faces challenges in handling complex scientific software that demands domain expertise, advanced software engineering practices, and intricate user workflows, due to the token limits and attention capabilities of current large language models (LLMs). To address these challenges, this paper presents a knowledge-driven framework that leverages knowledge representations in software engineering, scientific data, simulations, and software stacks to instruct and fine-tune Generative Pre-trained Transformers (GPT). This enables an autonomous software development workflow for generating code for sophisticated web applications, such as CyberGIS dashboards and visual analytics interfaces, from user-defined GUI wireframes sketched in PowerPoint or other graphical design tools (e.g., Adobe Illustrator). The prototyping workflow was implemented in Python using cutting-edge Generative AI and software engineering technologies, including the ChatGPT API and a local Ollama instance, within a RAG (Retrieval-Augmented Generation) paradigm that leverages Knowledge Graphs (KG) and vector databases. We demonstrate the feasibility and effectiveness of our framework through a case study that autonomously created a web-based platform that entails multiple visualization dashboards of environmental and energy data (e.g., time-series and spatial) based on user-defined visual prompts. The platform was built following industry-standard software engineering practices, such as Single-Page Application (SPA) and Model-View-ViewModel (MVVM) architecture patterns, that are modular, generalizable, reusable, and maintainable. Our work demonstrates the potential to reduce manual software design, coding, and maintenance efforts by guiding GenAI with software engineering knowledge, pioneering an autonomous and scalable approach for generating complex web applications to facilitate urban and environmental management within the smart city initiatives

In the past decades, scientific web applications (Web Apps), such as CyberGIS systems, visual analytical dashboards, digital twin platforms, and online decision support systems, have become indispensable tools for enabling both the scientific community and the public to discover, query, visualize, and download vast amounts of urban and environmental datasets in smart city research \citep{ferre2022adoption, dembski2020urban}. Aligned with the NSF's cyberinfrastructure (CI) initiative, academia and governmental science agencies have increasingly developed and adopted web applications as part of interdisciplinary informatics projects to serve as effective, user-friendly tools for cyber-delivery \citep{yu2021coevolution}. With advancements in internet and communication technologies, computing hardware, and artificial intelligence, these tools are transforming urban and environmental research by enabling data- and simulation-driven insights for decision support and optimization\citep{kadupitige2022enhancing}, fostering collaborative research through data and simulation sharing and integration \citep{parashar2019virtual}, and enhancing education and public engagement for citizen science and voluntary data collection \citep{skarlatidou2019volunteers} across various smart city disciplines. Notable application disciplines include water resources management \citep{souffront2018cyberinfrastructure, xu2022overview}, hazard mitigation \citep{mandal2024prime, xu2020web, garg2018cloud}, intelligent transportation systems \citep{xu2023smart, xu2022interactive, ghosh2017intelligent}, connected and automated vehicles\citep{xu2023mobile, kampmann2019dynamic}, built-environment management \citep{jia2019adopting, kim2022design}, and urban planning and design \citep{alatalo2017two}. Numerous interdisciplinary studies have demonstrated the transformative and unique capabilities of these scientific web applications in advancing environmental and urban research, as well as smart city management. Their continuous evolution is driven by the integration of emerging technologies such as artificial intelligence, the Internet of Things (IoT), edge computing, and cyber-physical systems. 

Despite the significant advancements in developing scientific web applications, creating customized software tools, such as cyberGIS and digital twin platforms for integrating and visualizing diverse types of environmental or urban data, such as hydrological data, traffic flow data, meteorological data, or simulation outputs, remains a highly demanding and resource-intensive task \citep{shanjun2024design, siddiqui2024digital, lei2023challenges}. These efforts require not only substantial expertise in software engineering and data engineering, but also considerable time spent on both client-side and server-side development, as well as database management, real-time data analytics, machine learning integration, and simulations \citep{ikegwu2022big}. As a result, urban and environmental researchers are often diverted from their core scientific and analytical work to learn complex web programming languages, frameworks, visualization libraries, UI/UX design principles, and database technologies \citep{li2022bibliometric}. Although modern software engineering practices, such as design patterns and architecture patterns, aim to streamline development and ensure maintainability, their effective use still requires specialized knowledge in software engineering \citep{fayad2015software}. Researchers, who may have programming expertise in data analytics but often lack formal software development experience, face challenges in applying these practices effectively \citep{kim2017data}. Even with the involvement of skilled software engineers, designing, developing, deploying, and maintaining large-scale scientific web applications remains a labor-intensive process, requiring repetitive and costly efforts \citep{shah2024optimizing, mcbreen2002software}. This hinders the scalability, flexibility, and adaptability of platforms like cyberGIS or digital twins, limiting their ability to incorporate new data types, extend to larger geographic regions, or enhance predictive analytics and decision support capabilities \citep{liu2015cybergis, lei2023challenges}. Given these challenges, there is a growing need to leverage emerging Generative AI (GenAI) technologies to automate various aspects of web application development to support environmental and urban research. Many contemporary studies have explored the potential and feasibility of training generative AI models, particularly Large Language Models (LLMs) and specialized variants like Generative Pretrained Transformers (GPT), to act as software developers by generating code for automating simple data analytics and software development tasks \citep{liang2024can, liukko2024chatgpt}. However, developing complex scientific web apps, such as cyberGIS platforms for querying and visualizing domain-specific environmental data across multiple sites, remains challenging. These challenges arise from the inefficiency and lack of systematic and graphical prompting methods, as well as the limitations in domain and software engineering knowledge, and attention mechanisms within current LLMs that are pre-trained using generalized text data.

==> Backup/backup_lit.tex <==

\subsection{The Raise of Transformer-based Language Models}

\subsection{Review of LLM in Software Engineering}
\citep{hou2023large} provides a comprehensive review of how large language models (LLMs) are being applied in software engineering (SE). The paper categorizes LLMs into different architectures such as encoder-only, encoder-decoder, and decoder-only models and analyzes their applications across various SE tasks like requirements engineering, code generation, bug fixing, program repair, and vulnerability detection. One of the key contributions is identifying the growing trend of using decoder-only models (e.g., GPT series) for automating code generation and completion tasks, showcasing their capability in reducing manual coding effort. However, challenges remain, including handling domain-specific knowledge, improving dataset quality, and managing the complexity of SE tasks that require more than simple text generation. The paper highlights the need for better preprocessing of data, fine-tuning of models for specific SE tasks, and the importance of using diverse datasets, particularly from industrial contexts, which are currently underrepresented in research. Future work proposes addressing these challenges through more focused studies on dataset variety, improving the robustness of LLMs in handling complex SE tasks, and refining evaluation metrics for assessing LLM performance in real-world SE environments. This paper significantly contributes to the field by providing a roadmap for future research in automating software development using LLMs, emphasizing the potential of these models to assist but not yet fully replace human developers in complex SE processes. 

\citet{fan2023large} provides an in-depth overview of how large language models (LLMs) like GPT, BERT, and Codex are being integrated into various software engineering tasks such as code generation, program repair, and automated testing. The paper identifies significant contributions to the automation of software development through generative AI, particularly in areas like automated code completion, bug detection, and software refactoring. It highlights how LLMs have revolutionized these tasks by reducing the manual effort required, improving coding efficiency, and enhancing developer productivity. However, the paper also notes several challenges, such as LLMs’ tendency to produce hallucinations (i.e., incorrect but plausible outputs), difficulties with domain-specific tasks, and the need for fine-tuning models to better suit specific software engineering contexts. It also mentions the problem of non-deterministic outputs from LLMs, which complicates scientific evaluation. Furthermore, the oracle problem persists in evaluating the correctness of generated solutions. The authors propose several areas for future work, including improving prompt engineering, hybridizing LLMs with traditional software engineering methods, and further research into how LLMs can be applied to underexplored areas like requirements engineering and software design. The integration of automated testing techniques with LLM outputs is also suggested as a way to mitigate hallucination and improve overall reliability.

\subsection{Evaluating LLM for Software Development}

\citet{liang2024can} explores the potential of GPT-4, a large language model (LLM), to replicate empirical software engineering research by identifying key assumptions and generating code for analysis pipelines. Through a user study involving 14 participants and seven empirical software engineering papers, the study found that GPT-4 could successfully surface correct assumptions, but it struggled with common knowledge and relevance, often lacking domain-specific expertise in software engineering. Although GPT-4 generated high-level analysis plans that accurately outlined research methodologies, the code it produced frequently contained errors such as incorrect data sources, missing steps, and implementation-level mistakes. Only 30\% of the generated code was executable without modifications. Despite these limitations, the study highlights GPT-4’s ability to provide a useful scaffold for automating parts of the software engineering process, particularly in replicating studies and creating analysis pipelines. GPT-4 can assist with brainstorming assumptions and structuring analysis code, potentially accelerating software development. However, due to its limitations, human oversight remains crucial for correcting errors and ensuring the accuracy and reliability of the generated code.
\citep{sandberg2024evaluating} investigates GPT-4’s ability to automate the development of full-stack web applications, examining both front-end and back-end generation. The study evaluates three web applications of varying complexity and analyzes key metrics such as prompt efficiency, debugging effort, and code quality. The findings highlight that GPT-4 can successfully generate functional applications, offering the advantage of speeding up the development process, especially for simpler projects. However, as application complexity increases, the tool struggles with debugging and handling intricate integrations, requiring significant human intervention. While GPT-4 can effectively generate foundational code, its limitations in dealing with complex logic, debugging, and quality assurance present notable challenges. This study underscores GPT-4’s role as a valuable assistant in automating parts of software development but not as a fully autonomous solution for complex systems, where human expertise remains essential.

\subsection{Existing GenAI Applications for Software Engineering}


\citep{phan2024hyperagent} introduces a novel multi-agent system designed to address a wide variety of software engineering (SE) tasks. HyperAgent consists of specialized agents (Planner, Navigator, Code Editor, and Executor) that mimic typical developer workflows, managing tasks from planning to execution. Through extensive evaluations on diverse benchmarks (SWE-Bench, RepoExec, and Defects4J), the system demonstrated superior performance in tasks such as GitHub issue resolution, repository-level code generation, and fault localization. HyperAgent significantly improves task success rates, outperforming specialized systems, particularly in complex, multi-step SE tasks across different programming languages. In terms of automating software development using generative AI, the key contribution of HyperAgent is its ability to autonomously handle large-scale, complex coding tasks, including bug fixing, feature addition, and program repair. The system’s use of LLMs across various subtasks showcases how generative AI can enhance automation in SE by reducing the need for manual intervention, especially in navigation, code editing, and execution. However, the paper also highlights several challenges, such as ensuring scalability across different programming environments and managing the computational cost of multi-agent coordination. Limitations include the potential for performance bottlenecks when handling larger codebases and debugging complex issues in real-time environments. Future work proposed in the paper involves integrating HyperAgent with version control systems, enhancing its explainability, and further refining the system to handle more specialized SE domains like security and performance optimization. These improvements could extend its applicability and make it a more practical tool for real-world software development.
\citep{xia2024agentless} challenges the need for complex, autonomous software engineering agents by introducing a simplified approach called AGENTLESS. This approach automates software development tasks, such as bug fixing, using a two-phase process: localization and repair. Unlike existing agent-based systems, which involve complex tool integration and autonomous decision-making, AGENTLESS employs a more straightforward hierarchical process for fault localization followed by patch generation. The paper demonstrates that this agentless approach can solve repository-level software issues with greater cost efficiency and competitive performance compared to state-of-the-art agent-based methods, achieving the highest performance on the SWE-bench Lite benchmark (27.33\%) at a fraction of the cost. Contribution to automating software development using generative AI: AGENTLESS leverages large language models (LLMs) to effectively automate bug localization and repair, offering a simpler yet robust alternative to more complex autonomous agents in software development. By removing the need for intricate tool management and decision-making mechanisms, the approach reduces complexity and improves interpretability. Challenges and Limitations: While AGENTLESS outperforms many open-source approaches, the paper identifies limitations such as reduced performance in scenarios where no localization clues are provided and difficulties in solving problems that require advanced reasoning or complex planning. Additionally, it highlights the need for improved re-ranking and selection techniques to maximize its repair capabilities. Future Work: The authors propose extending the AGENTLESS framework to address more complex software engineering tasks and to improve its problem-solving capabilities through better integration with testing frameworks and enhanced patch selection mechanisms. The paper contributes to the discourse on automating software development by emphasizing the potential of simpler, interpretable AI-driven methods over more complex autonomous agents.

\subsection{Code Generation}
\citep{gu2023effectiveness} provides a detailed empirical study on how large language models (LLMs) like ChatGPT, CodeLlama, and PolyCoder perform in domain-specific code generation tasks, focusing on the fields of web and game development. The authors reveal that while LLMs have shown great success in general-purpose code generation, their performance in domain-specific scenarios degrades significantly. This is largely due to the limited proficiency of these models in handling domain-specific libraries and APIs, resulting in issues such as API misuse and missing API calls. To address these challenges, the paper proposes DomCoder, a novel approach that integrates domain knowledge into LLMs through API recommendations and chain-of-thought prompting strategies. DomCoder shows improved performance across various domain-specific benchmarks, demonstrating the importance of enhancing LLMs with domain-specific prompts and fine-tuning for better results. 
Contribution to Automating Software Development using Generative AI: The paper's key contribution lies in showing how generative AI, when fine-tuned with domain-specific knowledge, can improve the automation of software development tasks, particularly in highly specialized domains such as game and web development. The integration of API knowledge into LLMs significantly enhances code generation performance, suggesting practical applications for automating more complex and specialized software engineering tasks. 
Challenges and Limitations: One major limitation is the scarcity of domain-specific data, which impacts the LLMs’ ability to fully learn the intricacies of domain-specific libraries. Additionally, integrating domain knowledge through complex APIs and prompts increases the difficulty of maintaining consistency and correctness in the generated code. 
Future Work: The authors propose future research directions, including improving LLM training with a richer variety of domain-specific datasets and enhancing prompt design mechanisms to further bridge the gap between general-purpose LLMs and domain-specific requirements. They also suggest exploring more sophisticated knowledge integration techniques, such as fine-tuning models with domain-relevant workflows and patterns to improve performance in complex domains.

\citep{zhang2023planning} introduces a novel approach called Planning-Guided Transformer Decoding (PG-TD), which improves the performance of large language models (LLMs) in code generation tasks by integrating a planning algorithm with Transformer models. Unlike traditional sampling and beam search methods, which rely on generating code first and then evaluating it, PG-TD incorporates a lookahead search that allows the model to make informed decisions during the generation process. This approach enables the model to generate higher-quality programs by considering test case results while the code is being generated. The method significantly improves pass rates on public competitive programming benchmarks compared to baseline methods.
Contribution to automating software development using generative AI: The introduction of PG-TD contributes to automating software development by optimizing code generation and reducing the need for extensive post-generation evaluation. It provides a more efficient way of generating programs that pass more test cases and is model-agnostic, meaning it can work with various Transformer-based LLMs without needing additional data or fine-tuning. 
Challenges and limitations: One of the key challenges of this approach is its reliance on available test cases for evaluating the quality of generated programs. The method is also more computationally expensive than simpler Transformer-based approaches due to the iterative tree search mechanism. Additionally, while it shows clear improvements in competitive programming scenarios, its effectiveness in broader software development contexts has not been fully explored. Future work: The authors propose improving the computational efficiency of PG-TD by exploring parallel tree search techniques and incorporating neural value functions to estimate pass rates more effectively. They also suggest extending the framework to support automatically generated test cases, addressing the issue of missing test cases in real-world scenarios. This paper makes a significant contribution to the ongoing development of generative AI in software engineering by enhancing the accuracy and efficiency of LLM-driven code generation.

\subsection{Knowledge Gaps}

\begin{description} 
   \item[Lack of Domain Knowledge] 
   \item[Hallucination] 
\end{description}

==> Sections/00_AAid.tex <==
This research presents a system-based approach to automate the software development of sophisticated GIS-based web applications to facilitate the urban and environmental management in smart city research, using ontology-driven prompts and ChatGPT, a widely used large language model (LLM). Our approach aims to leverage the AI model's generative, reasoning, and learning capability to create a primitive autonomous agent that helps academia researchers and would-be developers lower the technical barrier and cost to developing cyberinfrastructure and scientific software tools. At the technical level, we implemented a prototyping framework that employ a Knowledge Graph (KG) as the digital representation of software engineering practices, popular application stacks, and domain science knowledge to generate, tune, and enhance the engineered prompts through iterative procedures, creating accurate instructions to guide ChatGPT 4.0 API and LangChain to automate the development of a web-based geo-visual dashboards using widely-used frameworks and technologies favored by the industry. We demonstrate the performance and feasibility of our framework through a case of an AI-generated web applications. Through this study, we explore the LLM's potential as a full-stack web developer and GIS analyst trained by scientific knowledge graph to utilize advanced software design and architecture patterns (e.g., MVC and MVVM) and complex scientific data () to produce robust web app on both the server- and client-side. 

==> Sections/backup/0._Abstract.tex <==
Detecting and analyzing complex patterns in multivariate time series data is critical for informed decision-making in urban and environmental system operations. However, the high dimensionality, complexity, and interconnected nature of temporal patterns present significant challenges, particularly in understanding their underlying physical processes. Existing AI methods often struggle with limitations in interpretability, computational efficiency, and scalability, which undermine their trustworthiness and applicability in real-world scenarios.
To address these challenges, this paper proposes a novel visual analytics framework that reduces and interprets complex patterns in multivariate time series data through a combination of Time Fusion Transformer (TFT) and Variational Autoencoders (VAEs). The framework maps high-dimensional data into lower-dimensional latent spaces, which are further visualized in two-dimensional space using dimensionality reduction techniques such as PCA, t-SNE, and UMAP. These visualizations are enhanced through interactive multivariate displays and coordinated views, enabling researchers to explore pattern similarities using distance metrics. This approach uncovers potential correlations and topologies between patterns, improving the interpretability of generative models and facilitating exploratory fault pattern analysis.
The proposed framework is demonstrated through a case study on power grid signal data, where it effectively identifies grid event signatures—distinctive patterns indicative of faults and abnormal behaviors, such as capacitor switching, load shedding, and inverter malfunctions, as well as their potential interrelationships. Additionally, the framework incorporates novel metrics and visualizations to evaluate the performance, efficiency, and consistency of latent maps generated by TFT and VAE under varying configurations. This analysis provides valuable insights into model parameter tuning and enhances reliability. Comparative results show that TFT achieves shorter run times and better scalability to diverse data shapes compared to VAE.
This work pioneers the integration of TFT with visual analytics, advancing fault diagnosis in multivariate time series data. By fostering an explainable AI approach, it enhances decision-making processes in critical system operations, bridging the gap between AI-driven analysis and practical applicability.



==> Sections/backup/1._Intro.tex <==
\section{Introduction}
\label{Introduction}
Exploring patterns in multivariate time-series data is challenging due to the inherent complexity, heterogeneity, and high dimensionality of many environmental and urban datasets \citep{catley2008multi}. These datasets often involve multiple variables (i.e., features) measured over time, each interacting in non-linear ways and across different time scales \citep{goswami2019brief}. The temporal dependencies, varying trends, and potential noise within the data further complicate the task of identifying meaningful patterns, which may imply specific physical phenomena and events in real-world urban and environmental systems. Additionally, missing data points and irregular sampling intervals can hinder the accurate analysis of such data \citep{weerakody2021review, sun2020review}. To address these challenges, various AI-driven methods have been developed to enhance the classification and clustering of multivariate time-series data \citep{rojat2021explainable}. These approaches encompass a broad spectrum of techniques, ranging from traditional machine learning models like Principal Component Analysis (PCA) \citep{li2019multivariate} and Self-Organizing Maps (SOM) \citep{d2014wavelet}, to more advanced deep learning frameworks. Examples of these deep learning models include Recurrent Neural Networks (RNNs) \citep{ienco2020deep, wang2016effective} and Long Short-Term Memory (LSTM) networks \citep{karim2019multivariate, hong2017multivariate}, which excel in capturing temporal dependencies. Additionally, Convolutional Neural Networks (CNNs) have been successfully employed to identify both spatial and temporal patterns in multivariate time-series data \citep{liu2018time, tripathi2020multivariate}.Recently, generative algorithms, particularly Transformer models \citep{liu2021gated, zuo2023svp, le2024shapeformer, zerveas2021transformer}, have been increasingly employed for their ability to effectively model long-range dependencies in sequential data, making them highly suitable for tasks involving multivariate time-series analysis \citep{zhou2021informer}. Another popular generative AI model that was increasingly adopted to support multivariate time-series clustering is the Variational Autoencoder (VAE), which can effective facilitate missing data imputation and anomaly detection \citep{graving2020vae, lafabregue2022end, pham2022mst, yokkampon2022robust}. These deep generative models are able to learn the data distributions on high dimensional data spaces via a mapping to lower dimensional latent spaces.

However, despite advancements in AI-based methods, there remains a need to develop human-in-the-loop (HitL) approaches that allow for interaction and interpretation of insights generated by these models \citep{kumar2024applications, gomez2024human}. Human involvement is essential for validating AI-generated patterns and ensuring their relevance to specific domains \citep{tocchetti2022role}. For example, in power system operations, grid event signature data often involves complex multivariate time-series data, capturing various measurements—such as voltage, frequency, and current—across different time points \citep{wilson2024grid}. Discovering, interpreting, and understanding these grid signatures is crucial for ensuring reliable and efficient grid operations. These signatures represent distinct patterns or anomalies that could indicate system faults, operational inefficiencies, or potential disruptions \citep{rivas2020faults}. Events such as load shedding or inverter-based resource anomalies, for instance, can significantly impact grid stability if not properly understood and addressed \citep{das2024modeling, wilson2024grid}. In the context of operating urban systems, such as a power grid, the interpretation of these event patterns is critical for timely decision-making, making human involvement essential. While AI and automated systems can detect faults and anomalies, human expertise is required to validate, interpret, and apply these insights within the context of real-world urban system operations, such as power grid management. This interaction between human operators and AI systems underscores the importance of explainable AI (XAI) methods that provide greater transparency and interpretability, empowering grid operators to confidently act on insights derived from complex time-series data \citep{nallakaruppan2024advancing}. Meanwhile, visual analytics can further enhance human-AI interactions by helping users better understand deep learning models through interactive and intuitive visualizations and user interaction techniques, underscoring the importance of incorporating visual analytics methods into XAI methodologies.

 To address the challenges of interpretability in fault diagnosis for urban and environmental energy systems, this paper introduces a visual analytics framework designed to enhance the transparency and reliability of AI-driven operations in operating complex urban system. The framework integrates latent vector visualizations produced by Variational Autoencoders (VAEs) with coordinated, interactive visual encoding, clustering and highlighting complex patterns in multivariate time series data for more efficient interpretation. In a case study involving power grid signal data, we demonstrate how this framework enables the exploration of power grid event signatures, such as capacitor switching, load shedding, and inverter malfunctions, to facilitate fault diagnoses in urban power systems. Implemented into an interactive online visual analytical dashboard that is directly connected to the Grid Event Signature Library (GESL), our framework places HitL interactions at the heart of the Interactive Machine Learning (IML) and data-driven decision support processes. By bridging human expertise with black-box AI models, this approach supports data-informed decision-making, training, and educational activities in smart grid operations. The proposed method is also adaptable to other urban and environmental datasets, advancing visual analytics-powered explainable AI methods for more reliable and transparent system management.

%nd Local Interpretable Model-Agnostic Explanations (LIME) 

%Explainable AI methods allow users to understand model decision-making processes, which is crucial for building trust and enabling practical applications in real-world scenarios. %Integrating XAI techniques enhances transparency and interpretability in clustering, classification, and pattern extraction tasks within multivariate time-series data. 
 
% Through a case study that analyze power grid data, we demonstrate our method's capability in detecting grid signature events to support the identification, monitoring, and explortary analysis of abnormal behaviors critical for ensuring power system reliability and enabling timely interventions. 


 

==> Sections/backup/2._LitReview.tex <==
\section{Literature Review}
\label{Literature Review}
Exploring patterns in multivariate time-series data, which are inherently complex due to their high dimensionality, demands interdisciplinary approaches for effective decision support and operational applications. To structure our literature review, we divide it into four sections. The first two sections identifies key research needs for multivariate pattern analysis in prior urban and environmental studies, as well as smart grid operations. We review the relevant research applications in the grid operation sectors, as the grid data measured from various types of sensors and meters are often multivariate and provides a perfect real-world pattern exploration and analysis use case for fault diagnosis. Building on these needs, the second section reviews state-of-the-art methods that utilize AI and Human-in-the-Loop (HitL) approaches for dimensionality reduction, enabling experts to visually explore and interpret patterns in complex datasets. The third section highlights challenges that current methods face when assisting experts in visually analyzing patterns within multivariate time-series data. Using power grid signal data as a practical case, we identify knowledge gaps and outline the motivation and contributions of our study.

\subsection{Multivariate Pattern Detection and Exploration in Broad Urban Management Applications}
Exploring multivariate patterns in urban and environmental data, often used as surrogates to reflect underlying physical processes, is essential for the operation and management of various smart city systems. This approach is particularly valuable for generating new hypotheses, as well as facilitating anomaly detection and fault diagnosis \citep{erhan2021smart, sarker2022smart}. In practical smart city applications, analyzing the spatial and temporal variability across multiple environmental attributes, infrastructure features, and urban characteristics enables urban planners and environmental scientists to gain a deeper understanding of the complex, interconnected processes underlying various urban and environmental systems, such as transportation \citep{berres2021multiscale, pack2010visualization}, building energy \citep{xu2022geo, cottafava2018explorative}, public health \citep{xu2021episemblevis, preim2020survey}, and watershed management \citep{xu2022overview}. The empirical knowledge and data-driven insights gained from analyzing these patterns can then be leveraged to develop holistic and effective management practices, ultimately enhancing the operations, sustainability, and resilience of built environments \citep{bibri2021data}.

To highlight the importance of interpreting multivariate data pattern, we first review a handful of previous studies in the environmental and urban management sectors. \citet{xu2020web} introduces a web-based geovisual analytics platform that utilizes machine learning and visual analytics to address culvert sedimentation challenges, a significant infrastructure issue in watershed management. The platform integrates multiple data sources to analyze environmental variables impacting sedimentation, such as landscape and structural characteristics of culverts. By employing a tree-based feature selection algorithm and self-organizing maps (SOMs), the system identifies key sedimentation drivers and visualizes patterns from multivariate infrastructure and environment characteristics, thereby enabling users to explore spatial and relational data to locate sedimentation-prone regions and understand influencing factors. This tool assists in planning effective sediment mitigation strategies, facilitating informed decision-making for watershed and infrastructure managers, and offers a scalable explainable AI solution that is adaptable to broader environmental issues through the analysis of the multivariate geospatial data. In the transportation sector, \citet{dadashova2021multivariate} presents an advanced multivariate time series analysis to examine how socioeconomic factors influence urban traffic congestion. Using data from 51 U.S. metropolitan areas over a four-year period, the researchers identify key external drivers of congestion, including employment rates, rental vacancy rates, fuel prices, and building permits. These socioeconomic variables are incorporated into vector autoregressive models with exogenous factors (VAR-X), allowing for a robust prediction of congestion metrics such as travel time, planning time, and congested hours. The findings underscore the significant role of socioeconomic conditions in shaping traffic patterns, offering urban planners and transportation agencies valuable insights to improve traffic forecasting and implement targeted, data-informed congestion management strategies. The inherent explainability and interpretability of VAR models make them powerful tools for analyzing linear time-series data.
\citet{sanhudo2021multivariate} explores the use of machine learning for enhancing building energy management through multivariate time series analysis and clustering techniques. By applying k-medoids clustering and dynamic time warping to weather station data, the study creates clusters of meteorological conditions to improve data quality control and forecasting. Regression models, particularly Artificial Neural Networks (ANN) and Support Vector Regression (SVR), are then used to rectify missing or erroneous weather data, which is essential for reliable energy simulations. This data-driven approach proves effective, with ANNs slightly outperforming SVR in accuracy. The results demonstrate the potential for improved building energy efficiency by leveraging high-quality environmental data, supporting informed decision-making in energy retrofitting and optimization efforts. Although ANN and SVR offer automated pattern extraction, they are often considered partially interpretable with limited explainability, which restricts their capacity to help researchers gain deeper insights into the underlying patterns.
, \citet{hsieh2004nonlinear} explores advanced neural network methods for nonlinear multivariate and time series analysis, emphasizing their utility in fields like geophysics and environmental science. By extending classical methods such as Principal Component Analysis (PCA) and Canonical Correlation Analysis (CCA) to nonlinear versions (NLPCA and NLCCA), the research demonstrates how neural networks can reveal intricate patterns and dynamics that traditional linear models might miss. These nonlinear techniques, applied to climate and oceanographic data, allow for more accurate and insightful modeling of complex systems such as El Niño and the quasi-biennial oscillation. This research contributes valuable tools for managing and analyzing multivariate data in smart grid systems, where capturing non-linear patterns is crucial for adaptive and resilient infrastructure management.

Based on these example studies, it can be concluded that in various fields of urban and environmental studies, analyzing multivariate spatial and time-series data supports researchers and decision-makers in several key ways:
\begin{description} 
    \item [Perform dimensionality reduction] to cluster features based on multivariate similarity to cluster complex data, helping to identify environmental or urban phenomena based on specific attributes of one or more data features \citep{xu2020web, sanhudo2021multivariate}.
    \item [Investigate dependencies] between time series of multiple variables, enabling causal inferences about the underlying physical processes represented by these data variables \citep{dadashova2021multivariate}. 
\end{description}
By analyzing surrogate data to gain a deeper understanding of specific environmental or urban phenomena, as well as the correlations and dependencies between multiple physical processes within urban and environmental systems, researchers can leverage these insights to establish effective management practices. This approach enables the promotion or prevention of certain phenomena and their underlying processes, thereby helping to mitigate potential hazards and faults in urban systems.

\subsection{Multivariate Pattern Detection and Exploration in Grid Operations}
As a critical urban subsystem, smart grids produces vast amounts of multivariate and time-series data from a range of devices and sensors produce critical multivariate time series data. Smart meters installed at consumer sites record variables like power consumption, voltage, and frequency at intervals, providing insight into energy usage patterns. Phasor Measurement Units (PMUs), or synchrophasors, are positioned at substations to capture high-frequency measurements of voltage, current, and phase angle, aiding in real-time stability monitoring. SCADA systems, which aggregate data from Remote Terminal Units (RTUs) and Intelligent Electronic Devices (IEDs) across substations, monitor essential variables like voltage, current, power flow, and equipment status, creating continuous time series that reflect grid health. Additionally, Distributed Energy Resources (DERs), including solar panels and wind turbines, produce data on generation levels, voltage, and frequency, essential for integrating renewable energy. Environmental sensors contribute by capturing weather-related variables—temperature, humidity, wind speed—that impact demand and supply predictions. Together, these devices produce rich, multivariate time series data streams that enable comprehensive analysis and control of grid operations.

As examples, \citet{ceci2020echad} introduces ECHAD (Embedding-based CHAnge Detection), an unsupervised machine learning approach for smart grid management that uses embeddings and one-class learning to detect shifts in multivariate time series data, such as energy metrics. ECHAD dynamically adapts to new data patterns in real time, enhancing its resilience to collinearity and noise in complex sensor data. This method is particularly suited for monitoring renewable energy fluctuations and varying power loads, ensuring grid stability and efficiency. With high accuracy in detecting subtle and significant changes, ECHAD offers a robust tool for optimizing smart grid operations, although its reliance on embeddings and one-class learning may limit explainability. \citet{pinzon2019real} presents a real-time method for short-term voltage stability (STVS) assessment in power systems, using multivariate data from Phasor Measurement Units (PMUs) in Wide Area Monitoring Systems (WAMS). The approach employs a Random Forest (RF) model with symbolic discretization to classify time series data, identifying states under disturbances like fast voltage collapses (FVC) and fault-induced delayed voltage recovery (FIDVR). Features like the maximal Lyapunov exponent enable early instability detection, and the RF classifier provides interpretable alerts for voltage instability, aiding real-time decision-making. While effective for pre-defined labels (normal, alert, emergency, unstable), the model is limited in detecting new, unlabeled patterns, which restricts its use in adaptive, real-time fault diagnosis.

Multivariate pattern analysis in the grid operation sectors often emphasis the 
 

%Urban and environmental systems involve diverse data streams—such as air quality, population density, land use, and energy consumption—that influence each other in significant ways. By applying visual analytics, stakeholders can better discern patterns, correlations, and trends within this multivariate data, leading to more informed decision-making. For instance, understanding how air pollution levels are influenced by traffic patterns or industrial zones allows city planners to create strategies that mitigate health risks. Visual tools further enable dynamic exploration, making it easier for decision-makers to test scenarios, forecast outcomes, and communicate findings effectively. This data-driven insight is essential for developing sustainable urban policies, efficient resource management, and resilience against environmental challenges, ultimately leading to more responsive, adaptable urban and environmental systems.


\subsection{Latent Space Cartography and Visualization}
Deep generative models are universal tools for learning data distributions on high dimensional data spaces via a mapping to lower dimensional latent spaces.



\subsection{Knowledge Gaps and Motivation}


\section{Literature Review}
\label{Literature Review}
Analyzing patterns in multivariate time-series data, characterized by high dimensionality and complexity, requires interdisciplinary approaches to support effective decision-making. This literature review is structured into four sections. First, it identifies research needs for multivariate pattern analysis in urban and environmental studies. Second, it examines applications in power grid operations, where inherently multivariate data from diverse sensors provide practical use cases for fault diagnosis and pattern analysis. Third, it reviews AI and Human-in-the-Loop (HitL) methods for dimensionality reduction, enabling visual exploration and interpretation of complex datasets. Finally, it addresses challenges in current applications, emphasizing limitations in supporting experts with complex multivariate time-series data. Using power grid signal data as a case study, this review identifies knowledge gaps and drives advancements in fault diagnosis and multivariate pattern analysis.

\subsection{Multivariate Pattern Detection and Exploration in Broad Urban Management Applications}
Exploring multivariate patterns in urban and environmental data, often surrogates for underlying physical processes, is crucial for managing smart city systems. This approach supports hypothesis generation, anomaly detection, and fault diagnosis \citep{erhan2021smart, sarker2022smart}. By analyzing spatial and temporal variability across environmental attributes, infrastructure features, and urban characteristics, urban planners and environmental scientists can uncover insights into complex, interconnected systems such as transportation \citep{berres2021multiscale, pack2010visualization}, building energy \citep{xu2022geo, cottafava2018explorative}, public health \citep{xu2021episemblevis, preim2020survey}, and watershed management \citep{xu2022overview}. These insights drive the development of holistic management practices, enhancing the sustainability, resilience, and efficiency of urban environments \citep{bibri2021data}. 

To emphasize the importance of interpreting multivariate data patterns, we review notable studies in environmental and urban management. \citet{xu2020web} developed a web-based geovisual analytics platform leveraging machine learning and visual analytics to address culvert sedimentation, a key infrastructure issue in watershed management. The platform integrates diverse data sources and uses a tree-based feature selection algorithm and self-organizing maps (SOMs) to identify sedimentation drivers, visualize multivariate patterns, and inform mitigation strategies. This scalable, explainable AI tool is adaptable to broader environmental challenges. In the transportation sector, \citet{dadashova2021multivariate} used multivariate time series analysis to explore how socioeconomic factors impact urban traffic congestion. Using data from 51 U.S. metropolitan areas, they incorporated variables such as employment rates and fuel prices into vector autoregressive models with exogenous factors (VAR-X). These models provided interpretable insights for forecasting congestion metrics and informing targeted, data-driven management strategies. \citet{sanhudo2021multivariate} applied machine learning to improve building energy management through clustering and regression techniques. By using k-medoids clustering and dynamic time warping to enhance weather data quality, and Artificial Neural Networks (ANN) and Support Vector Regression (SVR) to rectify errors, the study demonstrated significant potential for energy optimization. However, limited explainability of these models restricts deeper insights into underlying patterns. Finally, \citet{hsieh2004nonlinear} extended classical techniques like PCA and CCA to nonlinear variants (NLPCA and NLCCA) using neural networks. Applied to climate and oceanographic data, these methods revealed intricate patterns in complex systems such as El Niño, offering valuable tools for managing multivariate data in smart grid systems and other resilient infrastructure applications.

Based on these example studies, it can be concluded that in various fields of urban and environmental studies, analyzing multivariate spatial and time-series data supports researchers and decision-makers in several key ways:
\begin{description}
    \item [Perform Dimensionality] reduction to group features based on multivariate similarities, facilitating the clustering of complex data. This approach aids in identifying environmental or urban phenomena by analyzing specific attributes of one or more data features \citep{xu2020web, sanhudo2021multivariate}. 
    \item [Explore Dependencies] among time series of multiple variables to enable causal inference, providing insights into the underlying physical processes represented by these data variables \citep{dadashova2021multivariate}.
\end{description}  
By analyzing surrogate data to understand environmental or urban phenomena and the interdependencies between physical processes, researchers can derive insights to inform effective management practices. This approach facilitates the promotion or mitigation of specific phenomena and their underlying processes, reducing potential hazards and faults in urban systems.

\subsection{Multivariate Pattern Detection and Exploration in Grid Operations}
As a critical urban subsystem, smart grids generate vast amounts of multivariate time-series data from various devices and sensors\citep{syed2020smart}. Smart meters at consumer sites record variables such as power consumption, voltage, and frequency, offering insights into energy usage patterns\citep{wang2020smart}. Phasor Measurement Units (PMUs) at substations capture high-frequency measurements like voltage, current, and phase angle, enabling real-time stability monitoring\citep{biswal2023real}. SCADA systems aggregate data from Remote Terminal Units (RTUs) and Intelligent Electronic Devices (IEDs) across substations, continuously monitoring grid health through variables like voltage, current, power flow, and equipment status \citep{manoj2021power}. Distributed Energy Resources (DERs), including solar and wind energy systems, provide data on generation levels, voltage, and frequency, which are critical for renewable energy integration. Environmental sensors add weather-related data—temperature, humidity, and wind speed—essential for predicting energy demand and supply \citep{nyangon2024climate}. Together, these data streams enable comprehensive grid analysis and control.

In the past decades, advanced time-series classification methods have been adopted into many power grid as a critical component of their monitoring and controls systems to facilitate anomaly detection, root cause analysis, and control purposes \citep{susto2018time}. 
For instance, \citet{ceci2020echad} introduces ECHAD (Embedding-based CHAnge Detection), an unsupervised machine learning method for detecting shifts in multivariate time-series data, such as energy metrics. ECHAD adapts dynamically to real-time patterns, improving resilience to collinearity and noise while monitoring renewable energy fluctuations and power loads. Although robust, its reliance on embeddings and one-class learning limits explainability. Similarly, \citet{pinzon2019real} proposes a Random Forest (RF)-based method for short-term voltage stability (STVS) assessment using PMU data. By classifying voltage states under disturbances like fast voltage collapses, the model provides interpretable alerts, aiding real-time decision-making. However, its reliance on predefined labels restricts its adaptability to new, unlabeled patterns.
\citet{alaca2024cnn} introduce a two-step phase fault classification method for analyzing power grid data using convolutional neural networks (CNNs). The first step involves fault detection, determining if a fault exists in the signal, while the second step identifies fault types, such as single-line-to-ground or line-to-line faults. Various feature extraction techniques, including amplitude and phase (AP), fast Fourier transform (FFT), wavelet transform (WT), and power spectral density (PSD), were explored to optimize performance. The study demonstrates that combinations like AP-AP and FFT-WT yield the highest accuracy. Simulation and real-world tests validate the method’s superiority over conventional one-step classification, highlighting its potential for real-time fault analysis in smart grid systems. 
\citep{bakdi2021real} introduces a novel data-driven methodology for analyzing multivariate time series data in grid-connected photovoltaic (GPV) systems. It employs Principal Component Analysis (PCA) for dimensionality reduction and decorrelation, followed by Kullback-Leibler Divergence (KLD) to detect anomalies. Kernel Density Estimation (KDE) refines the density estimation of transformed components (TCs) derived from PCA, enabling nonparametric and adaptive fault detection. This approach overcomes limitations of Gaussian assumptions, computational complexity, and parametric constraints. The methodology is validated through extensive experiments with real-world faults under Maximum and Intermediate Power Point Tracking (MPPT/IPPT) modes, demonstrating improved detection sensitivity, computational efficiency, and robustness to varying environmental conditions. Despite its high accuracy, both the methods are primarily designed to classify phase faults, rather than enabling an interactive ways to help domain experts explore and analyze different types of faults, and their potential connections.

Multivariate temporal pattern analysis in grid operation sectors often focuses on detecting data anomalies in continuous streams from devices such as Phasor Measurement Units (PMUs) and smart meters to extract operational insights and support decision-making. These analyses aim to enhance Fault Detection and Isolation (FDI), Predictive Maintenance, and Cybersecurity in grid management \citep{susto2018time}. However, practical grid management faces several challenges, including:

\begin{description} 
\item [Heterogeneous Data Sources:] Diverse data-generating systems and devices produce information in varying formats, structures, sampling rates, and resolutions. This diversity necessitates integration and standardization to enable meaningful analysis and actionable insights. 
\item [Nonstationary Signals:] Time-series data with statistical properties—such as mean, variance, and autocorrelation—that change over time, reflecting dynamic and evolving system behaviors rather than remaining constant. 
\item [High Computational Complexity:] Significant processing power and time are required to analyze large-scale, high-dimensional, and continuous data streams within stringent time constraints, which is essential for applications demanding immediate decision-making. 
\item [Scalability in Handling Vast Data Streams:] The ability of algorithms and systems to efficiently process and analyze massive, continuous flows of data from distributed sources, ensuring consistent performance and accuracy as data volume and velocity increase. 
\item [Noisy Data:] Power system signals are often affected by noise from environmental factors, equipment malfunctions, or communication errors. Noise can distort patterns, leading to misclassifications unless robust noise-filtering mechanisms are applied. 
\item [Missing Data:] Data gaps caused by sensor failures, communication issues, or maintenance downtimes can disrupt analysis. Classification algorithms must address these gaps without degrading performance through techniques such as imputation, interpolation, or robust model designs. 
\end{description}
These challenges underscore the need for developing intelligent methods that leverage emerging generative AI technologies. Such methods must be scalable to accommodate various types and dimensions of grid time series data while maintaining computational efficiency to support real-time analysis of large volumes of grid data, enabling near-instantaneous decision-making during grid operations.


\subsection{Latent Space Cartography and Visual Analytics}
Deep generative models serve as universal tools for learning data distributions in high-dimensional spaces by mapping them to lower-dimensional latent spaces, enabling efficient representation and synthesis of complex data patterns \citep{frenzel2019latent}. To increase the explainability and interprebility of these deep generative models and their outputs, a few recent studies have provided methodologies to visualize the latent representations of the complex high-dimension data. The latent representation is a compressed, lower-dimensional encoding of input data that is produced by generative AI models captures its essential features and structures while discarding irrelevant details, it can carry valuable information to help researcher explains how the AI models proceeds the complex data and produce the analytical outputs, such as clusters and classifications. Methodologies presented through these studies are often known as the "latent cartography", and have been developed to extract and analyze various types of data, emphasizing the interpretability and practical utility of latent spaces in diverse domains. 

As examples, \citet{frenzel2019latent} proposed metric-based transformations designed to improve the geometric structure of latent spaces generated by deep generative models, such as Variational Autoencoders (VAEs) and Generative Adversarial Networks (GANs). Their approach targets a significant gap in ensuring that latent space distances accurately represent semantic relationships, particularly in high-dimensional, non-Euclidean data like those encountered in natural language processing. This method enables enhanced clustering and interpolation, which are critical for applications such as language modeling and feature synthesis. \citet{liu2019latent} developed the concept of "Latent Space Cartography," an integrated visual analytics framework that facilitates tasks such as analogy construction, semantic dimension mapping, and latent space comparison. Designed for diverse datasets, including emojis, word embeddings, and biological features, their system employs user-defined semantic axes and advanced projection strategies, such as t-SNE and PCA, to uncover nuanced relationships within the data. By enabling interactive exploration, it bridges the gap between static visualizations and actionable insights, making it particularly valuable for scientific feature analysis and machine learning evaluation. \citet{kwon2023latent} introduced the "Latent Space Explorer," a multimodal visualization tool tailored for datasets such as cardiac MRIs and ECGs. This system provides a comprehensive workflow that integrates subgroup exploration, interactive decoding, and phenotype prediction accuracy analysis. By addressing the challenges of multimodal latent representation, the tool supports domain experts in uncovering subgroup-specific correlations and testing biases, thus enhancing clinical applications in cardiovascular health. \citet{o2022latent} further extended the latent space visualization paradigm by incorporating non-Euclidean geometries and multi-task metric learning to disentangle complex subgroup features in dynamic systems. Their methodology uses cartographic techniques to display latent spaces as two-dimensional visualizations, enabling users to examine patterns, correlations, and subgroup behaviors within fine-grained datasets. Applications include biological processes, where latent spaces reveal dynamic relationships affected by temporal or environmental factors, and physical systems, where domain knowledge informs geometric transformations for more robust interpretability.

These methodologies collectively address critical gaps in latent space analysis, including improving interpretability, maintaining geometric coherence, and supporting specific data modalities. They highlight the importance of tailored visualization tools for extracting meaningful insights from complex data, fostering advancements in AI-driven exploratory analysis across scientific, medical, and industrial domains.

\subsection{Knowledge Gaps and Motivation}
Desipte 
